GAN'SDA Wrap: Geographic And Network Structured Data on surfaces that Wrap around

There are many methods for projecting spherical maps onto the plane. Interactive versions of these projections allow the user to centre the region of interest. However, the effects of such interaction have not previously been evaluated. In a study with 120 participants we find interaction provides significantly more accurate area, direction and distance estimation in such projections. The surface of 3D sphere and torus topologies provides a continuous surface for uninterrupted network layout. But how best to project spherical network layouts to 2D screens has not been studied, nor have such spherical network projections been compared to torus projections. Using the most successful interactive sphere projections from our first study, we compare spherical, standard and toroidal layouts of networks for cluster and path following tasks with 96 participants, finding benefits for both spherical and toroidal layouts over standard network layouts in terms of accuracy for cluster understanding tasks.

==> sections/discussion.tex <==
\section{Discussion}
\begin{itemize}
    \item The results of our first study comparing readability of spherical projection of world maps indicate that with interaction, most projections significantly improve participants' error rate but is slower than static map projections.
    \item Our map study results also indicate that hemisphere maps tended to outperform non-hemisphere map projections in terms of error but is slower than non-hemisphere projections.
    \item Inspired by the results of the first study, we chose one non-hemisphere projection (\tequalearth{}) and one hemisphere projection (\torthographic{}) and compare them with standard and toroidal projections of node-link diagrams over their 2D projections of 3D geometry.
    \item For cluster identification tasks we find that all of toroidal and spherical equal earth and orthographic projections outperform traditional flat network layout, while toroidal and spherical equal earth outperform orthographic projection.
    \item To our surprise, while the results from Study 1 showed that \torthographic{} projections tended to be more accurate than non-hemisphere for error rate, it turned out to be significantly worse than \ttorus{} and \tequalearth{} for the second study comparing spherical projections of network clusters. Since \torthographic{} is an interrupted and non-area-preserving projection, it could be in fact turned out hard for participants to make out the network cluster boundaries when it is interrupted across the edge of the maps. 
    \item Though \torthographic{} performed quite well in Study 1, during our pilot studies of cluster tasks it reveal that the cut of clusters across two hemispheres and the strong distortion of clusters near the border of the Orthographic hemisphere made it hard for participants to count clusters. In fact, the shape of the cluster boundary may appear much larger than the small area size (how large and small, give a ratio) we use for study 1. 
    \item For network data, since the broken links may add cognitive load to participant, automatic panning that centres content of interest, such as high-level network structure, at the centre is important. For example, moving diagrams may involve mental load: \emph{``The ability to move the diagrams increased my likelyhood of mistakes, especially with an image where I could move and not know exactly where it begins or ends.''} and automatic pan reduced the need to pan: \emph{``The equal earth even though if we move the picture is very hard to understand the clusters, turned out to be the easiest to find the clusters (by not moving the picture).''}
    \item While we do not find any other related work on the visual analytics components such as area-preserving, distance, direction-preserving, that implies the design criteria of node-link diagrams on maps? The choice of map projections for the second study is inspired by the most successful results of the first map study.  E.g., why do we not draw straight line (as per normal node-link diagram) between nodes on a sphere but curved lines as geo-path? Is it because there will be much more link crossings?
    \item The paper by Jenny et al.~\cite{jenny2017force, jenny2018design} also mentioned angles are important for flow networks on maps. Is angle linked to any map tasks in our 1st study: distance/area/direction? Does our sphere layout have better incidence angle?
    \item Furthermore, they might easily get confused about links when they appear distorted or curved, as they need to take distortion and curved links into account. 
    \item Due to time limit, more analysis on the graph aesthetics of node-link diagrams on spherical projection evidence will be our next step.
    \item Our pilot results reveal that given the limited time to learn the interaction techniques and interact with the maps to find the answer, participants could easily got lost. Therefore, we provided them a strategy for the interactive conditions. This could be a possible reasons we don't see difference within round or flat maps. 
    \item It might be interesting to investigate, if in a lab-based supervised study where no time limit and nor any hint towards using the interactive techniques were given, whether participants would become more familiar with Orthographic than Mollweide within the round maps.
\end{itemize}
